Real-time Model Predictive Control and System Identification Using Differentiable Physics Simulation

Developing robot controllers in a simulated environment is advantageous but transferring the controllers to the target environment presents challenges, often referred to as the "sim-to-real gap". We present a method for continuous improvement of modeling and control after deploying the robot to a dynamically-changing target environment. We develop a differentiable physics simulation framework that performs online system identification and optimal control simultaneously, using the incoming observations from the target environment in real time. To ensure robust system identification against noisy observations, we devise an algorithm to assess the confidence of our estimated parameters, using numerical analysis of the dynamic equations. To ensure real-time optimal control, we adaptively schedule the optimization window in the future so that the optimized actions can be replenished faster than they are consumed, while staying as up-to-date with new sensor information as possible. The constant re-planning based on a constantly improved model allows the robot to swiftly adapt to the changing environment and utilize real-world data in the most sample-efficient way. Thanks to a fast differentiable physics simulator, the optimization for both system identification and control can be solved efficiently for robots operating in real time. We demonstrate our method on a set of examples in simulation and show that our results are favorable compared to baseline methods.

==> related_work_old.tex <==
\section{Related Work}
Deep reinforcement learning and model-based methods for robot control have both demonstrated impressive results in simulated environments. However, transferring controllers from simulated environment to real robot systems often fail due to the sim-to-real gap \citep{neunert2017off}, which has been an active research problem in recent years. Prior work has explored two different approaches to mitigate the sim-to-real gap: 1) Improving the accuracy and fidelity of robot models and simulators 2) Making the control policy more robust and adaptive to uncertainty or changes in system parameters.



\subsection{Improve modeling accuracy}
% Frequency response based sysid -> Model Based Parameter Optimization -> NeuralSim -> SimGAN
System identification (SysID) for robotic systems has been an important research area in robotics for decades. Classical methods for system identification, including the frequency response method and the impulse response method \cite{sysid_survey}, probe the system parameter offline using characteristic input signals. System parameters can also be identified by solving a regression problem for both linear systems \cite{RLS} and nonlinear ones \cite{NLRLS}. \textcolor{blue}{\cite{DOOMED} incrementally learns a linear model to compensate for the difference between dynamic equations and observations.} Offline SysID has been applied in identifying bending and stretching stiffness of cloth \cite{DiffCloth} and masses of articulated 2D multi-body systems \cite{LCP-Physics}. However, these methods cannot handle parameter change during control. For online SysID using incoming observations, recursive least square methods have been used for linear systems \cite{RLS}. Moreover, \cite{DUST, EMPPI} uses stochastic optimization to find current parameter from recent states. Recent development of learning-based approaches have attempted different directions in improving modeling accuracy and may allow us to model unknown time-varying components. For example, Yu \etal \cite{UP-OSI} learned a neural network to infer system parameters using recent sensor observations, which can model time varying parameters. Jiang \etal \cite{SimGAN} formulated system parameters as functions of state and action which can be learned from the real-world trajectories. Our adaptive system identification method is designed to run online and handle noisy state and action trajectories. Unlike learning-based methods, our online SysID does not require offline training using a large amount of data. 


%Another branch of classical methods formulate SysID as a regression problem. For linear system, these methods will solve linear least square regression to find the optimal parameters. To enable online update with new collected data, recursive least square method has been used in \cite{RLS}. To identify system parameter of non-linear system, regression based method need to solve a non-linear program which is not necessarily convex. However, by collecting enough data as well as utilizing gradient based optimization from deep learning field. Offline SysID has been applied in identifying bending and stretching stiffness of cloth \cite{DiffCloth} and masses of articulated 2D multi-body system\cite{LCP-Physics}.However, all of those methods can only identify constant system parameters. Recent development of learning based approach has attempt different direction in improving modeling accuracy and may allow us to model unknown time-varying component. \cite{UP-OSI} uses a neural network to infer system parameters using most recent observations, which can model time varying parameters. \cite{SimGAN} has proposed a force compensator can compensate unmodelled forces.

\subsection{Closing sim2real gap via controller design} % Whole subsection may need to be revised
% Need to read more content regarding traditional methods, for RL need to include some thing similar to UP-OSI.
% MRAC + MIT Rule (Each step will be a compensator optimized via gradient descent) They all assume strong linear assumption. (Our SSID Doesn't requires linear assumption)
%Designing more adaptive and robust controllers is an effective way to tackle sim-to-real problems. For linear systems, model reference adaptive control (MRAC) \cite{MRAC} aims to minimize model matching error by optimizing controller gains, or using a Lyapunov function to verify stability \cite{LypMRAC}. %In the robust control domain, Lyapunov functions \cite{CommonLyapunov} can be used to analyze a robust control policy, but Lyapunov function design for complex non-linear systems remains a challenging problem. 
% Recently, researchers have demonstrated that reinforcement learning can be an effective tool to learn robust or adaptive control policies. Domain randomization of simulation parameters has been used to transfer policies trained in simulation to different target environments \cite{DBLP:journals/corr/abs-1710-06537,DBLP:journals/corr/abs-1804-10332,DBLP:journals/corr/abs-1901-08652,DBLP:journals/corr/abs-2011-01891,DBLP:journals/corr/abs-1910-07113}. However, policies trained with domain randomization tend to trade off task performance for robustness, resulting in over-conservative behaviors \citep{DBLP:journals/corr/abs-1804-10332}. Learning adaptive control policies that can adjust behaviors for different environments using an estimation of the environment parameters is also a promising direction for sim-to-real transfer \cite{10.1162/153244303768966148,DBLP:journals/corr/HeessHLS15,DBLP:journals/corr/abs-2011-11270,UP-OSI,Peng20}. Our method is mostly related to Yu \etal \cite{UP-OSI} who proposed a method that trains a universal policy conditioned on the model parameters, which are identified by another learned system identification function. Our evaluation shows that our method achieves better task performance and system identification accuracy compared to the prior work.

\textcolor{blue}{Designing more adaptive and robust controller is an effective way to tackle sim-to-real problem. Robust control aims to design a controller that can control the system under inaccurate dynamics and noisy measurement. Common Lyapunov functions \cite{CommonLyapunov} can be used to verify controller's robustness, but finding a suitable Lyapunov function for complex non linear system is a challenging problem. More recently, domain and dynamic randomization have been used to transfer policies from simulation to different target environments\cite{DBLP:journals/corr/abs-1710-06537,DBLP:journals/corr/abs-1804-10332,DBLP:journals/corr/abs-1901-08652,DBLP:journals/corr/abs-2011-01891}. However, controllers design to be robust for different set of parameters have to trade off task performance. Alternatively ,in adaptive control, an online system identification identification module is used to update controller to adapt to different parameters. \cite{DUST, EMPPI} try to find the system parameters using stochastic optimization and update stochastic model predictive controller. \cite{UP-OSI, RMA} try to inference system parameters from history states using neural networks and feed the updated system parameter as part of state to a universal policy trained from reinforcement learning. Our method falls into the later category and it demonstrate superior performance compared with previous learning based or stochastic optimization based methods.}


\subsection{Differentiable physics}
In the last few years, various differentiable physics simulators have been proposed by researchers aiming to build better simulation tools for robotic tasks such as control, design and parameter identification. A significant amount of work focused on rigid body simulation \cite{kim2012lie,degrave2019differentiable,difftaichi,heiden2020augmenting,LCP-Physics,qiao2020scalable} with efficient formulations for contact \cite{geilinger2020add,nimble,Zhong2021NIPS,Qiao2021ICML,Xu2021RSS,Lidec2021ICRA} and constraints \cite{Lutter2021ICRA}. Soft body simulation has also been made differentiable \cite{schenck2018spnets,DiffCloth,hahn2019real2sim,hu2019chainqueen,qiao2020scalable,holl2020learning,geilinger2020add,DiSECT} and tested on different robotic tasks and hardware \cite{Wang2021IROS}. Roboticists have demonstrated that differentiable physics simulation can effectively identify simulation parameters \cite{degrave2019differentiable,difftaichi,Zhong2021NIPS,DiSECT,Wang2021IROS,Lidec2021ICRA}, optimize design parameters \cite{geilinger2020add,Xu2021RSS,Lutter2021ICRA}, or learn a hybrid simulator which combine learnable neural networks with differential equations \cite{heiden2020augmenting,ContactNets}. The gradient information can also be exploited in motion optimization \cite{nimble,DiSECT} and policy learning \cite{Qiao2021ICML,Zamora2021ICML}. The unique aspect of our method is that we utilize the gradients provided by a differentiable physics simulator simultaneously for control and system identification in an online fashion. This dual-purpose framework allows a robot to continue to adapt to an ever-changing environment in a sample efficient manner. 

% LCP-Physics -> Qiao Yiling's work -> Nimble
%In recent years, more and more differentiable simulators has been proposed by researchers aiming to build better simulation tools for robotics tasks such as control, design and parameter identification. \cite{LCP-Physics} was the first work that enable us to access analytical gradients and jacobians from 2D physics simulation with contact and experimented with offline mass identification and trajectory optimization problem on simple setups. Later on, \cite{DiffTaichi} implemented differentiable Material-Point-Method for soft body control problem and \cite{DiffCloth1,DiffCloth2} has enable differentiable differentiable cloth simulation which can be used for offline stiffness identification. \cite{nimble} built a feature complete differentiable simulator based on a popular simulator for robotics -- DART\cite{DART} and significantly accelerate the gradient computation with contact. Our work is built upon \cite{nimble} for convenience in setting up different environments and efficiency in computation.

